Benchmarking Stroke Forecasting with Stroke-Level Badminton Dataset

In recent years, badminton analytics has drawn attention due to the advancement of artificial intelligence and the efficiency of data collection. While there is a line of effective applications to improve and investigate player performance, there are only a few public badminton datasets that can be used by researchers outside the badminton domain. Existing badminton singles datasets focus on specific matchups; however, they cannot provide comprehensive studies on different players and various matchups. In this paper, we provide a badminton singles dataset, ShuttleSet22, which is collected from high-ranking matches in 2022. ShuttleSet22 consists of 30,172 strokes in 2,888 rallies in the training set, 1,400 strokes in 450 rallies in the validation set, and 2,040 strokes in 654 rallies in the testing set, with detailed stroke-level metadata within a rally. To benchmark existing work with ShuttleSet22, we hold a challenge, Track 2: Forecasting Future Turn-Based Strokes in Badminton Rallies, at CoachAI Badminton Challenge @ IJCAI 2023, to encourage researchers to tackle this real-world problem through innovative approaches and to summarize insights between the state-of-the-art baseline and improved techniques, exchanging inspiring ideas. The baseline codes and the dataset are made available at https://github.com/wywyWang/CoachAI-Projects/tree/main/CoachAI-Challenge-IJCAI2023.

==> table/data_columnname.tex <==
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
  
\begin{tabular}{c|c}
    \toprule
    Column Name & Explanation \\
    \midrule
    Rally & Serial number of rallies in a match.  \\
    \midrule
    Ball Round & The order of the shot in a rally. \\
    Time & The shot’s hitting time, which is in the format of hr:min:sec. \\
    Frame num & Equals to sec multiply fps. \\
    Round score A & Player A’s current score in the set. \\
    Round score B & Player B’s current score in the set. \\
    Player & The player who performed the shot. \\
    Type & The type of shot. \\
    Aroundhead & Hit the shuttle around the head or not. \\
    Backhand & Hit the shuttle with the backhand or not.  \\
    Landing height & If the shuttle destination is hit above (1) or below (0) the net. \\
    Landing area & The grid of the shuttle destinations \\
    \specialcell{Landing x \\Landing y} & The coordinates of the shuttle destinations. \\
    Reason for loss & The reason why the rally ended.\\
    Get the point player & The player who won the rally. \\
    Player location area & The location of the player who performed the shot.\\
    \specialcell{Player location x,\\Player location y} & The coordinates of the player’s location when the player hits the shuttle.\\
    Opponent location area & The location of the player who prepared to receive the shot.\\
    Opponent location x, Opponent location y & The coordinates of the opponent’s location when the player hits the shuttle. \\
    Set & The current set in a match (best-of-3).\\
    Match id & Serial number of matches \\
    Rally id & Serial number of all rallies\\
    Rally length & Number of shots in a rally, rally\_length-4 is the shots needed to predict. \\
    \bottomrule
\end{tabular}
  
% \begin{tabular}{c|cc}
%     \toprule
%     Column Name & Explanation & Data Type (Example) \\
%     \midrule
%     Rally & Serial number of rallies in a match. & Int \\
%     \midrule
%     Ball Round & The order of the shot in a rally. & Numerical \\
%     Time & The shot’s hitting time, which is in the format of hr:min:sec. & Str \\
%     Frame num & Equals to sec multiply fps. & Numerical \\
%     Round score A & Player A’s current score in the set. & Numerical \\
%     Round score B & Player B’s current score in the set. & Numerical \\
%     Player & The player who performed the shot. & Numerical \\
%     Type & The type of shot. & Category (Drive, Net Shot, Lob, Clear, Drop, Puch/Rush, Smash, Defensive Shot, Short Service, Long Service) \\
%     Aroundhead & Hit the shuttle around the head or not.  & Binary \\
%     Backhand & Hit the shuttle with the backhand or not. & Binary \\
%     Landing height & If the shuttle destination is hit above (1) or below (0) the net. & Binary \\
%     Landing area & The grid of the shuttle destinations & Category \\
%     \specialcell{Landing x,\\Landing y} & The coordinates of the shuttle destinations. & Numerical \\
%     Reason for loss & The reason why the rally ended. & Category\\
%     Get the point player & The player who won the rally. & Numerical \\
%     Player location area & The location of the player who performed the shot. & Category\\
%     \specialcell{Player location x,\\Player location y} & The coordinates of the player’s location when the player hits the shuttle. & Numerical\\
%     Opponent location area & The location of the player who prepared to receive the shot. & Category\\
%     Opponent location x, Opponent location y & The coordinates of the opponent’s location when the player hits the shuttle. & Numerical\\
%     Set & The current set in a match (best-of-3). & Numerical\\
%     Match id & Serial number of matches & Numerical\\
%     Rally id & Serial number of all rallies & Numerical\\
%     Rally length & Number of shots in a rally, rally\_length-4 is the shots needed to predict. & Numerical \\
%     \bottomrule
% \end{tabular}

==> table/lose_reason.tex <==
\begin{tabular}{c|c}
    \toprule
    Loss Reason & Count & Percent\\
    \midrule
    Opponent's ball landed & 701 &\\
    Out &&\\
    Touched the net &&\\
    Not pass over the net &&\\
    Misjudged & 81 &\\
    \bottomrule
\end{tabular}
